SPaR: Self-Play with Tree-Search Refinement to Improve Instruction-Following in Large Language Models

Instruction-following is a fundamental capability of language models, requiring the model to recognize even the most subtle requirements in the instructions and accurately reflect them in its output. Such an ability is well-suited for and often optimized by preference learning. However, existing methods often directly sample multiple independent responses from the model when creating preference pairs. Such practice can introduce content variations irrelevant to whether the instruction is precisely followed (e.g., different expressions about the same semantic), interfering with the goal of teaching models to recognize the key differences that lead to improved instruction following. In light of this, we introduce SPaR, a self-play framework integrating tree-search self-refinement to yield valid and comparable preference pairs free from distractions. By playing against itself, an LLM employs a tree-search strategy to refine its previous responses with respect to the instruction while minimizing unnecessary variations. Our experiments show that a LLaMA3-8B model, trained over three iterations guided by SPaR, surpasses GPT-4-Turbo on the IFEval benchmark without losing general capabilities. Furthermore, SPaR demonstrates promising scalability, greatly enhancing models like GLM-4-9B and LLaMA3-70B. We also identify how inference scaling in tree search would impact model performance. Our code and data are publicly available at https://github.com/thu-coai/SPaR.

==> sections/method.tex <==
% 整体思路
We introduce \model, an automatic and scalable method for effective self-evolution in instruction-following tasks. 
The core idea of our framework is to leverage the self-refinement capability of LLMs to produce response pairs, thereby highlighting the key differences that determine task success or failure and avoiding distractions (Figure \ref{fig: abs}).

The overall framework of our method is illustrated in Figure \ref{fig: method}. 
Our framework operates in a cyclical manner, with one model serving as the actor and another model serving dual roles as both judge and refiner. 
These models are initialized from the same base model to facilitate continuous self-improvement with the SFT dataset for different capabilities.

Specifically, due to the lack of high-quality multi-constraint instruction-following datasets, we start by using a taxonomy-based method to systematically create a diverse and complex set of instruction prompts (\S\ref{para: prompt creation}). 
Next, we equip the actor model with strong instruction-following skills and train the refiner to initially critique and refine the actor's responses (\S\ref{para: model initialization}).
During the iterative training process, the refiner analyzes the actor's responses, identifies errors (\S\ref{para: wrong response collection}), and utilizes tree-search algorithms to refine them (\S\ref{para: tree search refinemen}). This method produces a refined set of instruction-response pairs that highlight the subtle differences crucial for accurate instruction following.
Subsequently, we apply Direct Preference Optimization (DPO) to further train the actor model (\S\ref{para: actor dpo}). At the same time, the refiner model undergoes Rejection Sampling Fine-Tuning (RFT) to improve its evaluation and refinement capabilities (\S\ref{para: reinfer rft}).



\subsection{Data Construction}

\subsubsection{Prompt Creation} \label{para: prompt creation}
% 数据资源稀缺
Given the scarcity of high-quality data for instruction-following tasks, especially those with multiple constraints, we first create a high-quality dataset of instruction-following prompts.

\paragraph{Seed Prompts.}
To ensure the quality and diversity of our dataset, and to prevent issues like insufficient diversity or even model collapse \citep{liu2024best, shumailov2024ai}, we use a seed set of prompts derived from the Infinity-Instruct dataset \citep{zhao2024iidoptimizinginstructionlearning}, which contains ten million high-quality conversations. We focus on the \textit{commonsense} and \textit{subjective} subsets, excluding \textit{coding} and \textit{math} to avoid unreasonable instructions in subsequent steps. After applying rule-based filtering based on length, keywords, and self-BLEU, we obtain approximately 50k seed prompts.

% taxonomy-based构建，统计
\paragraph{Taxonomy-based Prompt Evolution.} Prompt evolution without human intervention tends to be poorly diversified, as the types of constraints added are often distributed unevenly and unreasonable \citep{sun2024conifer}. Therefore, we propose a taxonomy-based prompt evolution mechanism to make constraint types comprehensive and balanced.
Our taxonomy for instruction-following constraints is derived from \citet{cheng2024autodetect} and further refined to be more comprehensive.

After we build the constraint taxonomy, $T$, we conduct the prompt evolution to get complex instruction-following tasks. We sample a main constraint type $c_0$ and employ a strong LLM to add several other constraints $\{c_1, c_2, \ldots, c_N\}$ to complicate the original prompt. Formally, this process can be presented as $x = LLM(p, c_0, \ldots, c_N)$, where $p$ is the seed prompt and $x$ is the complex prompt.
The detailed taxonomy and prompt can be found in Appendix \ref{appendix: prompt and taxonomy}.

\subsubsection{Actor and Refiner Intialization} \label{para: model initialization}
Our taxonomy-based prompt evolution results in about 43k prompts. We utilize 8k prompts for actor initialization training, another 5k for the refiner, and save 30k for further iterative training. 

\paragraph{Actor Data Creation.} To bootstrap the actor model with strong instruction-following capabilities, we first distill a strong LLM's responses to these complex prompts, thereby producing supervised fine-tuning (SFT) data, $(x, y) \in D_\text{Actor}$. Then, we train the base model to get a strong actor, $M_{0}$.

\paragraph{Refiner Data Creation.} To bootstrap the refiner model with strong judgment and refinement capability, we sample several responses, $\{y_1, \ldots, y_N\}$, from the initial actor $M_0$. Then, we distill the judgment capability from a strong LLM to form a dataset, $(x, y, j) \in D_\text{JSFT}$.
We collect responses that are judged not to accurately follow instructions and define them as negative responses.
For these negative responses, we use the strong LLM to refine them to be correct with minimal revisions. 
In this way, we get a refinement dataset, $(x, y_\text{negative}, j, y_\text{refined}) \in D_\text{RSFT}$. The refiner is then trained with $D_\text{Refiner} = D_\text{JSFT} \cup D_\text{RSFT}$ to create the initial refiner, $R_0$.


\paragraph{Training Strategy.}
For both actor and refiner models, we use standard supervised fine-tuning with the loss function:
\begin{equation} \label{loss: SFT}
    \mathcal{L}=-\frac{1}{N}\sum_{t=1}^N\text{log}P(r_t|q,r_{<t}) 
\end{equation} 
Here, $q$ denotes the input, $r$ signifies the target response and $N$ represents the length of $r$.
% For actor training, $q=x, r=y$. As for the refiner, $q=(x,y), r=j$ for $D_{JSFT}$ and $q=(x,y_{wrong},j), r=y_\text{refined}$ for $D_{RSFT}$. 
For actor training, we have $q = x$ and $r = y$. When it comes to the refiner, we use $q = (x, y)$ and $r = j$ for $D_\text{JSFT}$, and $q = (x, y_\text{negative}, j)$ and $r = y_\text{refined}$ for $D_\text{RSFT}$.

\subsection{Iterative Self-refinement Training}
After initializing the actor and refiner models, we embark on an iterative process for continuous self-improvement.
In each iteration, we first gather the negative data, where the responses fail to accurately follow the instructions (\S\ref{para: wrong response collection}). Then, we utilize a tree-search algorithm to refine the negative responses (\S\ref{para: tree search refinemen}) and form the training data for the next actor (\S\ref{para: actor dpo}) and refiner (\S\ref{para: reinfer rft}).
This iterative pipeline allows us to continuously improve both models.

\subsubsection{Negative Data Collection} \label{para: wrong response collection}
For each prompt, $x$, we first sample $K$ responses $\{y_1, y_2, \ldots, y_K\}$ from the actor model. This step ensures that there are enough incorrect responses to support subsequent training. 
Then, we utilize the refiner to judge whether each response is correct. To make this judgment more accurate, we incorporate the self-consistency mechanism \citep{wang2022self}, which is also applied in the subsequent refinement process. 
Specifically, we obtain multiple judgments from the refiner and determine the final label through majority voting, as detailed in Appendix \ref{appendix: exp}. 
After majority voting, we randomly select one judgment that matches the voted label to serve as the final judgment.
This process allows us to identify challenging prompts that elicit incorrect responses, yielding tuples of the form $(x, y_\text{negative}, j)$, where $y_\text{negative}$ is the incorrect response and $j$ is its corresponding judgment. 


\subsubsection{Tree-search Refinement} \label{para: tree search refinemen} 
After collecting these negative instances, the next step is to refine the incorrect responses to form preference pairs. These pairs are crucial for highlighting the subtle distinctions that can determine the success of instruction-following tasks, thereby facilitating effective learning.
Given that direct refinement often results in a low success rate, we employ a tree-search approach. We implement both breadth-first search (BFS) and depth-first search (DFS) strategies for this refinement. Detailed algorithms for these methods are provided in Appendix \ref{appendix: tree search}.

To illustrate our process, we take BFS as an example. 
Starting with an incorrect instruction-response pair and its judgment as the root node, we expand the tree level-by-level until a correct response is found.
At each depth level, we generate potential refinements for the current set of responses and evaluate their correctness using the Refiner.
The number of generated refinements corresponds to the number of branches. Specifically, for each depth, the Refiner:
1). Generates potential refinements for each state in the current level; 2). Judges the correctness of these refinements. We then update the set of states with new responses and their corresponding judgments.
The iterative process continues until we obtain a tuple $(x, y_\text{negative}, j, y_\text{refined})$, where $y_\text{refined}$ is the newly refined, correct response.


% During this process, each extension involves two uses of the refiner: one to refine the response of the parent node, and another to self-judge whether the current refinement meets the complex instruction perfectly. This iterative process continues until we obtain a tuple $(x, y_{wrong}, j, y_\text{refined})$, where $y_\text{refined}$ is the newly refined, correct response.


\subsubsection{Actor Training} \label{para: actor dpo}
To optimize the actor model, we leverage the refinement pairs for preference learning using DPO.
In the $N_{th}$ iteration, we train the actor model $M_{N}$ with refinement pairs $(y_\text{negative}, y_\text{refined})$, treating $y_\text{negative}$ as the rejected response ($y_l$) and $y_\text{refined}$ as the chosen response ($y_w$). The training data is denoted as $D_{dpo}^{N}$.
The DPO loss can be represented as follows:
\begin{equation}
    \mathcal{L}_{\text{DPO}} (\pi_{\theta}^{\text{N}}; \pi_{\text{ref}}) = - \mathbb{E}_{(x, y_w, y_l) \sim D_{dpo}^{N}} \left[ \log \sigma \left( \beta \log \frac{\pi_{\theta}^{\text{N}} (y_w | x)}{\pi_{\text{ref}} (y_w | x)} - \beta \log \frac{\pi_{\theta}^{\text{N}} (y_l | x)}{\pi_{\text{ref}} (y_l | x)} \right) \right]
\end{equation}
Here, $\pi_{\theta}^N$ represents the actor model $M_N$, and the reference model $\pi_{ref}$ initialized with $M_N$ remains fixed during the training process. This results in a new actor model, $M_{N+1}$, for the next iteration.

\subsubsection{Refiner Training} \label{para: reinfer rft}
% Given that the input for the refiner is templated, we use RFT to train the new refiner, $R_{N+1}$. 
% The RFT dataset is comprised of training data for both judgement and refinement capabilities. 

% We denote the parent of the final node of the refinement tree as $(x, y_p, j_p)$. Then, the refinement dataset consists of tuples $(x, y_p, j_p, y_\text{refined}) \in D_{refine}^N$. The judgement dataset utilizes the majority-voting labels, represented as $(x, y_i, j_i) \in D_{judge}^N$. 
% Supervised fine-tuning is then performed using the loss equation \ref{loss: SFT},
% % \begin{equation}
% % \mathcal{L}=-\frac{1}{N}\sum_{t=1}^N\text{log}P(r_t|q,r_{<t}) 
% % \end{equation}
% with $q=(x, y_p, j_p), r=y_\text{refined}$ for $D_{refine}^N$ and $q=(x,y_i), r=j_i$ for $D_{judge}^N$. 

Given that the input for the refiner is templated, we use RFT to train the new refiner, $R_{N+1}$. 
The RFT training data consists of two components: the refinement data and the judgment data.

\paragraph{Refinement Training Data.} The refinement training data consists of tuples that capture the process of refining incorrect responses. For each incorrect response from the previous tree-search refinement step, we collect tuples of the form $(x, y_p, j_p, y_\text{refined})$, where $(x, y_{p}, j_{p})$ represents the parent node of the final correct response in the refinement tree, and $y_\text{refined}$ is the correctly refined response.

\paragraph{Judgment Training Data.} The judgment training data is derived both from the negative data collection and nodes of the tree-search process. This dataset consists of tuples $(x, y_i, j_i)$, where $x$ is the prompt, $y_i$ is a response to $x$, and $j_i$ is the judgment after majority voting.

Then, we perform supervised fine-tuning using the constructed training data. For the refinement data $D_\text{refine}^N$ we use the tuples $(x, y_p, j_p, y_\text{refined})$ with input $q=(x, y_p, j_p)$ and target $r=y_\text{refined}$. For the judgment data $D_\text{judge}^N$, we use the tuples $(x, y_i, j_i)$ with input $q=(x, y_i)$ and target $r=j_i$. The supervised fine-tuning loss is given by Equation \ref{loss: SFT}.

==> tables/ablation_llama.tex <==
\begin{table}[!t]
\centering

    \caption{Actor's ablation study on iteratively trained LLaMA3-8B-Instruct.}
    \vspace{1mm} 
    \renewcommand{\arraystretch}{1.2} % 调整行距
    \setlength{\tabcolsep}{1.0mm} % 调整列间距
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{IFEval}} & \textbf{FollowBench (SSR)} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4}
      & \textbf{Prompt(S)} & \textbf{Instruction(S)} & \textbf{Avg.} \\
    \midrule
    \model-DPO-iter3 & 78.0 & 83.7 & 68.8\\
    \midrule
    \textit{w/o} Tree Search & -2.0 & -0.8 & -1.7 \\
    \textit{w/o} Iterative Training & -0.9 & -0.2 & -2.0 \\
    \textit{w/o} Refinement & -2.6  & -1.6   & -3.1 \\
    \bottomrule
    \end{tabular}
\label{tab:actor_ablation_llama3}
\end{table}

==> tables/ablation_llama_judge.tex <==
\begin{table}[!t]
\centering

    \caption{Refiner's ablation study on iteratively trained LLaMA3-8B-Instruct.}
    \vspace{1mm} 
    \renewcommand{\arraystretch}{1.4} % 调整行距
    \setlength{\tabcolsep}{1.0mm} % 调整列间距
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Natural}} & \multicolumn{2}{c}{\textbf{Adversarial}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
      & Acc. & F1 & Acc. & F1 \\
    \midrule
    \model-DPO-iter3 & 70.5 & 65.9 & 67.8 & 62.4\\
    \midrule
    \textit{w/o} Tree Search & -0.5 & -1.2 & -4.3 & -8.2 \\
    \textit{w/o} Iterative Training & -0.5 & -2.5 & -1.7 & -3.5 \\
    \bottomrule
    \end{tabular}
\label{tab:refiner_ablation_llama3}
\end{table}

==> tables/general_ability_llama.tex <==
\begin{table}[ht]
% \begin{wraptable}{r}{0.75\textwidth}
\centering
\caption{Performance on general benchmarks for iteratively trained LLaMA3-8B-Instruct. \model maintains the model's general capabilities.}
\vspace{1mm}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cccc|l}
\toprule
\textbf{Model}     & \textbf{GSM8k} & \textbf{TriviaQA} & \textbf{MMLU} & \textbf{HumanEval} & \textbf{Average} \\ \midrule
LLaMA3-8B-Instruct & 75.4           & 75.9              & 63.6          & 55.5               & 67.6          \\ \midrule
\model-SFT                & 75.6           & 76.0                & 64.0            & 61.6               & 69.3 {\color{ForestGreen}\textsubscript{\textbf{(+1.7)}}}          \\ \midrule
\model-DPO-iter1               & 78.8          & 75.2              & 63.8          & 60.4               & 69.6 {\color{ForestGreen}\textsubscript{\textbf{(+2.0)}}}        \\ \midrule
\model-DPO-iter2               & 77.0             & 74.9              & 63.1          & 60.4               & 68.9  {\color{ForestGreen}\textsubscript{\textbf{(+1.3)}}}       \\ \midrule
\model-DPO-iter3               & 77.7           & 75.1              & 63.1          & 60.9               & 69.2  {\color{ForestGreen}\textsubscript{\textbf{(+1.6)}}}        \\ \bottomrule
\end{tabular}}
\label{tab: general ability} 
\end{table}

% \begin{wraptable}{r}{4.3cm}
% 	\centering
% 	\begin{tabular}{lrrr}
% 	%.....
% 	\end{tabular}
% \end{wraptable}

==> tables/general_reinfment.tex <==
\begin{table}[!t]
    \centering

    %------------------------------gpt4 ablation ------------------------------------------
    \begin{minipage}{0.65\textwidth}
    \tiny
    \centering
        \caption{Performance on general benchmarks for iteratively trained LLaMA3-8B-Instruct (Cf. Table \ref{tab: mistral general ability} for Mistral-7B-Instruct).}
    \renewcommand{\arraystretch}{1.0} % 修改行距
    \setlength{\tabcolsep}{1mm} % 设置单元格间距
    \resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\toprule
\textbf{Model}     & \textbf{GSM8k} & \textbf{TriviaQA} & \textbf{MMLU} & \textbf{HumanEval} & \textbf{Average} \\ \midrule
LLaMA3-8B-Instruct & 75.4           & 75.9              & 63.6          & 55.5               & 67.6          \\ \midrule
\model-SFT                & 75.6           & \textbf{76.0}                & \textbf{64.0}            & \textbf{61.6}               & 69.3          \\ \midrule
\model-DPO-iter1               & \textbf{78.8}           & 75.2              & 63.8          & 60.4               & \textbf{69.6}         \\ \midrule
\model-DPO-iter2               & 77.0             & 74.9              & 63.1          & 60.4               & 68.9         \\ \midrule
\model-DPO-iter3               & 77.7           & 75.1              & 63.1          & 60.9               & 69.2          \\ \bottomrule
\end{tabular}}
\label{tab: general ability} 
    
    \end{minipage}
    %-----------------------------------ablation specific component--------------------------
    \hfill
    \begin{minipage}{0.34\textwidth}
    \tiny
    \centering
        \caption{Refinement evaluation results. Acc-GPT uses GPT-4o as judge; -\model uses \model-RFT-iter3.}
    \renewcommand{\arraystretch}{0.95} % 调整行距
    \setlength{\tabcolsep}{1.0mm} % 调整列间距
    \label{tab:refine llama3}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c}
\toprule
\textbf{Model} & \textbf{Acc-GPT}  & \textbf{Acc-\model} \\ \midrule
GPT-4o-Mini        & \textbf{79.0} & 71.0  \\
\midrule
\model-SFT            & 73.5          & 71.0               \\ \midrule
\model-RFT-iter1           & 77.5          & 77.0               \\ \midrule
\model-RFT-iter2           & 74.5          & 76.0               \\ \midrule
\model-RFT-iter3           & \textbf{79.0} & \textbf{90.5}      \\ \bottomrule
\end{tabular}}
    \end{minipage}
    %-----------------------------------ablation specific component--------------------------
    \vspace{-3mm}
\end{table}
